Evolution Reinforces Cooperation with the Emergence of Self-Recognition Mechanisms: an empirical study of the Moran process for the iterated Prisoner's dilemma

We present insights and empirical results from an extensive numerical study of the evolutionary dynamics of the iterated prisoner's dilemma. Fixation probabilities for Moran processes are obtained for all pairs of 164 different strategies including classics such as TitForTat, zero determinant strategies, and many more sophisticated strategies. Players with long memories and sophisticated behaviours outperform many strategies that perform well in a two player setting. Moreover we introduce several strategies trained with evolutionary algorithms to excel at the Moran process. These strategies are excellent invaders and resistors of invasion and in some cases naturally evolve handshaking mechanisms to resist invasion. The best invaders were those trained to maximize total payoff while the best resistors invoke handshake mechanisms. This suggests that while maximizing individual payoff can lead to the evolution of cooperation through invasion, the relatively weak invasion resistance of payoff maximizing strategies are not as evolutionarily stable as strategies employing handshake mechanisms.

==> tex/summary_top_10_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                    CS &          0.7322 \\
2  &                   \textbf{TF2} &          0.7249 \\
3  &                   \textbf{TF1} &          0.7203 \\
4  &              Predator &          0.7046 \\
5  &              Prober 4 &          0.6895 \\
6  &             Handshake &          0.6848 \\
7  &               Grudger &          0.6633 \\
8  &                   \textbf{TF3} &          0.6611 \\
9  &                  MEM2 &          0.6602 \\
10 &                 Davis &          0.6580 \\
11 &          Fool Me Once &          0.6550 \\
12 &  EvolvedLookerUp1\_1\_1 &          0.6546 \\
13 &           Hard Prober &          0.6545 \\
14 &           Retaliate 3 &          0.6519 \\
15 &              Winner21 &          0.6492 \\
16 &           Retaliate 2 &          0.6474 \\
\bottomrule
\end{tabular}


==> tex/summary_top_10_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2274 \\
2  &        PSO Gambler 2\_2\_2 &      0.2223 \\
3  &     EvolvedLookerUp2\_2\_2 &      0.2203 \\
4  &              Evolved ANN &      0.2199 \\
5  &            Evolved ANN 5 &      0.2193 \\
6  &             Fool Me Once &      0.2174 \\
7  &        PSO Gambler 1\_1\_1 &      0.2147 \\
8  &            Evolved HMM 5 &      0.2145 \\
9  &  Evolved FSM 16 Noise 05 &      0.2141 \\
10 &                  Grudger &      0.2110 \\
11 &                     MEM2 &      0.2107 \\
12 &                      \textbf{TF3} &      0.2105 \\
13 &         PSO Gambler Mem1 &      0.2100 \\
14 &              Meta Hunter &      0.2099 \\
15 &            Evolved FSM 4 &      0.2081 \\
16 &                       CS &      0.2063 \\
\bottomrule
\end{tabular}


==> tex/summary_top_10_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9907 \\
2  &          \textbf{TF1} &          0.9879 \\
3  &          \textbf{TF2} &          0.9851 \\
4  &     Predator &          0.9841 \\
5  &     Prober 4 &          0.9731 \\
6  &    Handshake &          0.9719 \\
7  &     Winner21 &          0.9625 \\
8  &  Hard Prober &          0.9561 \\
9  &    Fortress4 &          0.9475 \\
10 &       Ripoff &          0.9456 \\
11 &       Tester &          0.9449 \\
12 &      Grudger &          0.9429 \\
13 &          \textbf{TF3} &          0.9422 \\
14 &        Davis &          0.9420 \\
15 &  Retaliate 3 &          0.9406 \\
16 &         MEM2 &          0.9404 \\
\bottomrule
\end{tabular}


==> tex/summary_top_11_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2339 \\
2  &        PSO Gambler 2\_2\_2 &      0.2293 \\
3  &              Evolved ANN &      0.2274 \\
4  &            Evolved ANN 5 &      0.2264 \\
5  &     EvolvedLookerUp2\_2\_2 &      0.2264 \\
6  &             Fool Me Once &      0.2238 \\
7  &            Evolved HMM 5 &      0.2221 \\
8  &        PSO Gambler 1\_1\_1 &      0.2214 \\
9  &  Evolved FSM 16 Noise 05 &      0.2208 \\
10 &         PSO Gambler Mem1 &      0.2164 \\
11 &            Evolved FSM 4 &      0.2156 \\
12 &                     MEM2 &      0.2153 \\
13 &                  Grudger &      0.2149 \\
14 &                      \textbf{TF3} &      0.2147 \\
15 &              Meta Hunter &      0.2142 \\
16 &                Omega TFT &      0.2118 \\
\bottomrule
\end{tabular}


==> tex/summary_top_11_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9898 \\
2  &          \textbf{TF1} &          0.9876 \\
3  &          \textbf{TF2} &          0.9854 \\
4  &     Predator &          0.9840 \\
5  &     Prober 4 &          0.9744 \\
6  &    Handshake &          0.9710 \\
7  &     Winner21 &          0.9610 \\
8  &  Hard Prober &          0.9554 \\
9  &    Fortress4 &          0.9536 \\
10 &       Ripoff &          0.9452 \\
11 &       Tester &          0.9444 \\
12 &      Grudger &          0.9387 \\
13 &          \textbf{TF3} &          0.9382 \\
14 &        Davis &          0.9382 \\
15 &  Retaliate 3 &          0.9365 \\
16 &         MEM2 &          0.9363 \\
\bottomrule
\end{tabular}


==> tex/summary_top_12_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                    CS &          0.7545 \\
2  &                   \textbf{TF2} &          0.7533 \\
3  &                   \textbf{TF1} &          0.7465 \\
4  &              Predator &          0.7273 \\
5  &              Prober 4 &          0.7142 \\
6  &             Handshake &          0.7059 \\
7  &               Grudger &          0.6804 \\
8  &                   \textbf{TF3} &          0.6788 \\
9  &                  MEM2 &          0.6775 \\
10 &                 Davis &          0.6753 \\
11 &           Hard Prober &          0.6745 \\
12 &              Winner21 &          0.6742 \\
13 &  EvolvedLookerUp1\_1\_1 &          0.6734 \\
14 &          Fool Me Once &          0.6730 \\
15 &           Retaliate 3 &          0.6709 \\
16 &     Forgetful Grudger &          0.6662 \\
\bottomrule
\end{tabular}


==> tex/summary_top_12_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2174 \\
2  &        PSO Gambler 2\_2\_2 &      0.2109 \\
3  &     EvolvedLookerUp2\_2\_2 &      0.2088 \\
4  &              Evolved ANN &      0.2083 \\
5  &            Evolved ANN 5 &      0.2066 \\
6  &            Evolved HMM 5 &      0.2038 \\
7  &             Fool Me Once &      0.2037 \\
8  &        PSO Gambler 1\_1\_1 &      0.2030 \\
9  &  Evolved FSM 16 Noise 05 &      0.2009 \\
10 &         PSO Gambler Mem1 &      0.1985 \\
11 &            Evolved FSM 4 &      0.1979 \\
12 &                     MEM2 &      0.1953 \\
13 &                      \textbf{TF3} &      0.1950 \\
14 &              Meta Hunter &      0.1948 \\
15 &                  Grudger &      0.1945 \\
16 &                Fortress4 &      0.1944 \\
\bottomrule
\end{tabular}


==> tex/summary_top_12_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9956 \\
2  &          \textbf{TF1} &          0.9933 \\
3  &          \textbf{TF2} &          0.9911 \\
4  &     Predator &          0.9898 \\
5  &     Prober 4 &          0.9821 \\
6  &    Handshake &          0.9775 \\
7  &     Winner21 &          0.9728 \\
8  &  Hard Prober &          0.9682 \\
9  &    Fortress4 &          0.9650 \\
10 &       Ripoff &          0.9608 \\
11 &       Tester &          0.9601 \\
12 &      Grudger &          0.9544 \\
13 &          \textbf{TF3} &          0.9540 \\
14 &        Davis &          0.9537 \\
15 &  Retaliate 3 &          0.9532 \\
16 &         MEM2 &          0.9526 \\
\bottomrule
\end{tabular}


==> tex/summary_top_13_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2231 \\
2  &        PSO Gambler 2\_2\_2 &      0.2176 \\
3  &     EvolvedLookerUp2\_2\_2 &      0.2145 \\
4  &              Evolved ANN &      0.2144 \\
5  &            Evolved ANN 5 &      0.2136 \\
6  &            Evolved HMM 5 &      0.2101 \\
7  &             Fool Me Once &      0.2094 \\
8  &        PSO Gambler 1\_1\_1 &      0.2091 \\
9  &  Evolved FSM 16 Noise 05 &      0.2077 \\
10 &            Evolved FSM 4 &      0.2048 \\
11 &         PSO Gambler Mem1 &      0.2048 \\
12 &              Meta Hunter &      0.2013 \\
13 &                      \textbf{TF3} &      0.1988 \\
14 &                     MEM2 &      0.1988 \\
15 &   Evolved ANN 5 Noise 05 &      0.1985 \\
16 &                Omega TFT &      0.1981 \\
\bottomrule
\end{tabular}


==> tex/summary_top_13_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9958 \\
2  &          \textbf{TF1} &          0.9947 \\
3  &          \textbf{TF2} &          0.9930 \\
4  &     Predator &          0.9909 \\
5  &     Prober 4 &          0.9824 \\
6  &    Handshake &          0.9777 \\
7  &     Winner21 &          0.9714 \\
8  &    Fortress4 &          0.9675 \\
9  &  Hard Prober &          0.9670 \\
10 &       Ripoff &          0.9585 \\
11 &       Tester &          0.9579 \\
12 &      Grudger &          0.9505 \\
13 &          \textbf{TF3} &          0.9502 \\
14 &        Davis &          0.9501 \\
15 &  Retaliate 3 &          0.9491 \\
16 &         MEM2 &          0.9485 \\
\bottomrule
\end{tabular}


==> tex/summary_top_14_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                   \textbf{TF2} &          0.7617 \\
2  &                    CS &          0.7563 \\
3  &                   \textbf{TF1} &          0.7510 \\
4  &              Predator &          0.7299 \\
5  &              Prober 4 &          0.7131 \\
6  &             Handshake &          0.7079 \\
7  &               Grudger &          0.6842 \\
8  &                   \textbf{TF3} &          0.6823 \\
9  &                  MEM2 &          0.6820 \\
10 &              Winner21 &          0.6798 \\
11 &           Hard Prober &          0.6797 \\
12 &  EvolvedLookerUp1\_1\_1 &          0.6790 \\
13 &                 Davis &          0.6786 \\
14 &          Fool Me Once &          0.6778 \\
15 &           Retaliate 3 &          0.6752 \\
16 &             Retaliate &          0.6718 \\
\bottomrule
\end{tabular}


==> tex/summary_top_4_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                    CS &          0.6676 \\
2  &              Predator &          0.6386 \\
3  &                   \textbf{TF1} &          0.6376 \\
4  &                   \textbf{TF2} &          0.6318 \\
5  &              Prober 4 &          0.6302 \\
6  &             Handshake &          0.6264 \\
7  &               Grudger &          0.6223 \\
8  &                   \textbf{TF3} &          0.6183 \\
9  &                  MEM2 &          0.6179 \\
10 &                 Davis &          0.6144 \\
11 &          Fool Me Once &          0.6125 \\
12 &  EvolvedLookerUp1\_1\_1 &          0.6038 \\
13 &           Hard Prober &          0.6030 \\
14 &           Retaliate 3 &          0.6026 \\
15 &         Evolved ANN 5 &          0.6010 \\
16 &           Evolved ANN &          0.6003 \\
\bottomrule
\end{tabular}


==> tex/summary_top_4_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &                  Grudger &      0.3568 \\
2  &                       CS &      0.3553 \\
3  &                     MEM2 &      0.3547 \\
4  &             Fool Me Once &      0.3537 \\
5  &                      \textbf{TF3} &      0.3533 \\
6  &           Evolved FSM 16 &      0.3503 \\
7  &            Evolved ANN 5 &      0.3490 \\
8  &              Evolved ANN &      0.3490 \\
9  &                    Davis &      0.3489 \\
10 &        PSO Gambler 2\_2\_2 &      0.3483 \\
11 &     EvolvedLookerUp2\_2\_2 &      0.3459 \\
12 &              Meta Hunter &      0.3450 \\
13 &  Evolved FSM 16 Noise 05 &      0.3445 \\
14 &        PSO Gambler 1\_1\_1 &      0.3435 \\
15 &     EvolvedLookerUp1\_1\_1 &      0.3421 \\
16 &                 Prober 4 &      0.3416 \\
\bottomrule
\end{tabular}


==> tex/summary_top_4_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &        Player &  Mean $p_{N-1}$ \\
\midrule
1  &            CS &          0.9084 \\
2  &           \textbf{TF1} &          0.8915 \\
3  &      Predator &          0.8895 \\
4  &           \textbf{TF2} &          0.8795 \\
5  &     Handshake &          0.8785 \\
6  &      Prober 4 &          0.8632 \\
7  &      Winner21 &          0.8371 \\
8  &   Hard Prober &          0.8319 \\
9  &       Grudger &          0.8279 \\
10 &           \textbf{TF3} &          0.8246 \\
11 &         Davis &          0.8229 \\
12 &          MEM2 &          0.8220 \\
13 &     Fortress4 &          0.8170 \\
14 &   Retaliate 3 &          0.8169 \\
15 &  Fool Me Once &          0.8161 \\
16 &   Retaliate 2 &          0.8133 \\
\bottomrule
\end{tabular}


==> tex/summary_top_5_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &                  Grudger &      0.3112 \\
2  &           Evolved FSM 16 &      0.3098 \\
3  &                     MEM2 &      0.3098 \\
4  &             Fool Me Once &      0.3096 \\
5  &                      \textbf{TF3} &      0.3090 \\
6  &        PSO Gambler 2\_2\_2 &      0.3058 \\
7  &              Evolved ANN &      0.3056 \\
8  &            Evolved ANN 5 &      0.3053 \\
9  &     EvolvedLookerUp2\_2\_2 &      0.3042 \\
10 &                    Davis &      0.3034 \\
11 &                       CS &      0.3027 \\
12 &        PSO Gambler 1\_1\_1 &      0.3019 \\
13 &              Meta Hunter &      0.3017 \\
14 &  Evolved FSM 16 Noise 05 &      0.3015 \\
15 &            Evolved HMM 5 &      0.2990 \\
16 &     EvolvedLookerUp1\_1\_1 &      0.2981 \\
\bottomrule
\end{tabular}


==> tex/summary_top_5_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &        Player &  Mean $p_{N-1}$ \\
\midrule
1  &            CS &          0.9416 \\
2  &           \textbf{TF1} &          0.9303 \\
3  &      Predator &          0.9263 \\
4  &           \textbf{TF2} &          0.9248 \\
5  &     Handshake &          0.9152 \\
6  &      Prober 4 &          0.9063 \\
7  &      Winner21 &          0.8841 \\
8  &   Hard Prober &          0.8772 \\
9  &       Grudger &          0.8664 \\
10 &     Fortress4 &          0.8652 \\
11 &           \textbf{TF3} &          0.8641 \\
12 &         Davis &          0.8637 \\
13 &          MEM2 &          0.8614 \\
14 &   Retaliate 3 &          0.8594 \\
15 &  Fool Me Once &          0.8569 \\
16 &   Retaliate 2 &          0.8566 \\
\bottomrule
\end{tabular}


==> tex/summary_top_6_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                    CS &          0.7068 \\
2  &                   \textbf{TF1} &          0.6845 \\
3  &                   \textbf{TF2} &          0.6823 \\
4  &              Predator &          0.6790 \\
5  &             Handshake &          0.6615 \\
6  &              Prober 4 &          0.6614 \\
7  &               Grudger &          0.6451 \\
8  &                   \textbf{TF3} &          0.6421 \\
9  &                  MEM2 &          0.6407 \\
10 &                 Davis &          0.6381 \\
11 &          Fool Me Once &          0.6340 \\
12 &  EvolvedLookerUp1\_1\_1 &          0.6300 \\
13 &           Hard Prober &          0.6296 \\
14 &           Retaliate 3 &          0.6286 \\
15 &           Retaliate 2 &          0.6236 \\
16 &   Limited Retaliate 3 &          0.6226 \\
\bottomrule
\end{tabular}


==> tex/summary_top_6_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2774 \\
2  &             Fool Me Once &      0.2737 \\
3  &                  Grudger &      0.2735 \\
4  &        PSO Gambler 2\_2\_2 &      0.2735 \\
5  &                     MEM2 &      0.2724 \\
6  &                      \textbf{TF3} &      0.2722 \\
7  &            Evolved ANN 5 &      0.2720 \\
8  &              Evolved ANN &      0.2720 \\
9  &                       CS &      0.2718 \\
10 &     EvolvedLookerUp2\_2\_2 &      0.2706 \\
11 &        PSO Gambler 1\_1\_1 &      0.2685 \\
12 &                    Davis &      0.2677 \\
13 &              Meta Hunter &      0.2677 \\
14 &  Evolved FSM 16 Noise 05 &      0.2663 \\
15 &            Evolved HMM 5 &      0.2646 \\
16 &     EvolvedLookerUp1\_1\_1 &      0.2640 \\
\bottomrule
\end{tabular}


==> tex/summary_top_6_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &               Player &  Mean $p_{N-1}$ \\
\midrule
1  &                   CS &          0.9627 \\
2  &                  \textbf{TF1} &          0.9549 \\
3  &             Predator &          0.9503 \\
4  &                  \textbf{TF2} &          0.9496 \\
5  &            Handshake &          0.9379 \\
6  &             Prober 4 &          0.9349 \\
7  &             Winner21 &          0.9185 \\
8  &          Hard Prober &          0.9107 \\
9  &              Grudger &          0.9005 \\
10 &            Fortress4 &          0.8999 \\
11 &                  \textbf{TF3} &          0.8988 \\
12 &                Davis &          0.8987 \\
13 &                 MEM2 &          0.8964 \\
14 &          Retaliate 3 &          0.8954 \\
15 &  Limited Retaliate 3 &          0.8933 \\
16 &          Retaliate 2 &          0.8933 \\
\bottomrule
\end{tabular}


==> tex/summary_top_8_coexist.tex <==
\begin{tabular}{llr}
\toprule
{} &                Player &  Mean $p_\{N/2\}$ \\
\midrule
1  &                    CS &          0.7275 \\
2  &                   \textbf{TF2} &          0.7119 \\
3  &                   \textbf{TF1} &          0.7116 \\
4  &              Predator &          0.6999 \\
5  &              Prober 4 &          0.6837 \\
6  &             Handshake &          0.6799 \\
7  &               Grudger &          0.6615 \\
8  &                   \textbf{TF3} &          0.6587 \\
9  &                  MEM2 &          0.6575 \\
10 &                 Davis &          0.6549 \\
11 &          Fool Me Once &          0.6521 \\
12 &  EvolvedLookerUp1\_1\_1 &          0.6489 \\
13 &           Hard Prober &          0.6484 \\
14 &           Retaliate 3 &          0.6462 \\
15 &           Retaliate 2 &          0.6417 \\
16 &     Forgetful Grudger &          0.6415 \\
\bottomrule
\end{tabular}


==> tex/summary_top_8_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2372 \\
2  &        PSO Gambler 2\_2\_2 &      0.2313 \\
3  &              Evolved ANN &      0.2292 \\
4  &             Fool Me Once &      0.2289 \\
5  &            Evolved ANN 5 &      0.2288 \\
6  &     EvolvedLookerUp2\_2\_2 &      0.2287 \\
7  &                  Grudger &      0.2248 \\
8  &            Evolved HMM 5 &      0.2243 \\
9  &        PSO Gambler 1\_1\_1 &      0.2241 \\
10 &                     MEM2 &      0.2238 \\
11 &                      \textbf{TF3} &      0.2237 \\
12 &  Evolved FSM 16 Noise 05 &      0.2235 \\
13 &                       CS &      0.2212 \\
14 &              Meta Hunter &      0.2209 \\
15 &         PSO Gambler Mem1 &      0.2185 \\
16 &                    Davis &      0.2182 \\
\bottomrule
\end{tabular}


==> tex/summary_top_8_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9851 \\
2  &          \textbf{TF1} &          0.9810 \\
3  &          \textbf{TF2} &          0.9773 \\
4  &     Predator &          0.9771 \\
5  &    Handshake &          0.9650 \\
6  &     Prober 4 &          0.9649 \\
7  &     Winner21 &          0.9518 \\
8  &  Hard Prober &          0.9462 \\
9  &    Fortress4 &          0.9394 \\
10 &       Ripoff &          0.9340 \\
11 &       Tester &          0.9333 \\
12 &      Grudger &          0.9332 \\
13 &          \textbf{TF3} &          0.9323 \\
14 &        Davis &          0.9321 \\
15 &         MEM2 &          0.9303 \\
16 &  Retaliate 3 &          0.9302 \\
\bottomrule
\end{tabular}


==> tex/summary_top_9_invade.tex <==
\begin{tabular}{llr}
\toprule
{} &                   Player &  Mean $p_1$ \\
\midrule
1  &           Evolved FSM 16 &      0.2444 \\
2  &        PSO Gambler 2\_2\_2 &      0.2398 \\
3  &              Evolved ANN &      0.2380 \\
4  &            Evolved ANN 5 &      0.2370 \\
5  &     EvolvedLookerUp2\_2\_2 &      0.2370 \\
6  &             Fool Me Once &      0.2356 \\
7  &            Evolved HMM 5 &      0.2328 \\
8  &        PSO Gambler 1\_1\_1 &      0.2327 \\
9  &  Evolved FSM 16 Noise 05 &      0.2320 \\
10 &                     MEM2 &      0.2290 \\
11 &                      \textbf{TF3} &      0.2286 \\
12 &                  Grudger &      0.2286 \\
13 &         PSO Gambler Mem1 &      0.2284 \\
14 &              Meta Hunter &      0.2276 \\
15 &            Evolved FSM 4 &      0.2255 \\
16 &                    Davis &      0.2237 \\
\bottomrule
\end{tabular}


==> tex/summary_top_9_resist.tex <==
\begin{tabular}{llr}
\toprule
{} &       Player &  Mean $p_{N-1}$ \\
\midrule
1  &           CS &          0.9859 \\
2  &          \textbf{TF1} &          0.9824 \\
3  &          \textbf{TF2} &          0.9780 \\
4  &     Predator &          0.9779 \\
5  &     Prober 4 &          0.9659 \\
6  &    Handshake &          0.9655 \\
7  &     Winner21 &          0.9508 \\
8  &  Hard Prober &          0.9433 \\
9  &    Fortress4 &          0.9369 \\
10 &       Ripoff &          0.9307 \\
11 &       Tester &          0.9298 \\
12 &      Grudger &          0.9280 \\
13 &        Davis &          0.9273 \\
14 &          \textbf{TF3} &          0.9271 \\
15 &         MEM2 &          0.9251 \\
16 &  Retaliate 3 &          0.9250 \\
\bottomrule
\end{tabular}

